The Decidability and Complexity of Interleaved Bidirected Dyck Reachability

Dyck reachability is the standard formulation of a large domain of static analyses, as it achieves the sweet spot between precision and efficiency, and has thus been studied extensively. Interleaved Dyck reachability (denoted $D_k\odot D_k$) uses two Dyck languages for increased precision (e.g., context and field sensitivity) but is well-known to be undecidable. As many static analyses yield a certain type of bidirected graphs, they give rise to interleaved bidirected Dyck reachability problems. Although these problems have seen numerous applications, their decidability and complexity has largely remained open. In a recent work, Li et al. made the first steps in this direction, showing that (i) $D_1\odot D_1$ reachability (i.e., when both Dyck languages are over a single parenthesis and act as counters) is computable in $O(n^7)$ time, while (ii) $D_k\odot D_k$ reachability is NP-hard. In this work we address the decidability and complexity of all variants of interleaved bidirected Dyck reachability. First, we show that $D_1\odot D_1$ reachability can be computed in $O(n^3\cdot \alpha(n))$ time, significantly improving over the existing $O(n^7)$ bound. Second, we show that $D_k\odot D_1$ reachability (i.e., when one language acts as a counter) is decidable, in contrast to the non-bidirected case where decidability is open. We further consider $D_k\odot D_1$ reachability where the counter remains linearly bounded. Our third result shows that this bounded variant can be solved in $O(n^2\cdot \alpha(n))$ time, while our fourth result shows that the problem has a (conditional) quadratic lower bound, and thus our upper bound is essentially optimal. Fifth, we show that full $D_k\odot D_k$ reachability is undecidable. This improves the recent NP-hardness lower-bound, and shows that the problem is equivalent to the non-bidirected case.

==> algorithms/algo_2n2n.tex <==
\smallskip
\begin{algorithm}%[H]
\small
\DontPrintSemicolon
%\SetInd{0.3em}{0.3em}
\caption{$\AlgoTwoN$}\label{algo:2n2n}
\KwIn{
A path $P\colon u\DODOPath v$, a $(1,2)$-positive cycle $C\colon x\Path x$, a path $Q\colon u\Path x$.
}
\KwOut{
A (non simple) cycle $Z\colon u\Path u$ that contains all cycles of $\Cycles(P)$.
}
\BlankLine
Let $c_i\gets \Counter_i(Q)$ for each $i\in[2]$\\
Let $Z\gets C$\\
Let $\Worklist\gets \Cycles(P)$\\
\While(\tcp*[f]{Step 1: Inflate both counters sufficiently}){$c_i<2\cdot n$ for some $i\in[2]$}{
$Z\gets Z\circ C$\\
$c_i\gets \Counter_i(C)$ for each $i\in [2]$
}
Let $j\gets\arg \min_{l} c_l$\tcp*[r]{The counter with the smallest value so far}
\While(\tcp*[f]{Step 2: Cycle elimination with }){$\exists H\in Z$ s.t. $\Counter_{3-j}(H)\geq 0$}{
\eIf{}{
}{
}
}
\Return{$Q$}
\end{algorithm}





==> algorithms/algo_bounded_path.tex <==
\smallskip
\begin{algorithm}%[H]
\small
\DontPrintSemicolon
%\SetInd{0.3em}{0.3em}
\caption{$\BoundedPathsAlgo$}\label{algo:bounded_paths}
\KwIn{
A path $P\colon u\DPath{\Dyck_1\odot \Dyck_1} v$, the subpath $P'\in \Prefixes(P)$ s.t.
\begin{compactenum}
\item $\Counter_1(P')=n$
\item $\Counter_i(P'')<n$ for every $i\in[2]$ and subpath $P''\in \Prefixes(P')$ with $|P''| <|P'|$
\end{compactenum}
}
\KwOut{A path $Q\colon u\DPath{\Dyck_1\odot \Dyck_1} v$ that satisfies the bounded-paths property}
\BlankLine
Let $Q\gets P'$
Let $S\gets P\setminus P'$\\
Let $L\gets \Cycles(P')$\\
Let $\Flag\gets \True$
\While{$\Flag$}{
$\Flag\gets\False$\\
\eIf{$\Counter_2(Q)\geq n$}{
\uIf{$L$ has a cycle $C'$ with $\Counter_1(C')\geq 0$ and $\Counter_2(C')\leq 0$}{
Let $C\gets$ the first such cycle\\
$\Flag\gets \True$\\
}
}{
\uIf{$S$ has a reachable cycle $C'$ with $\Counter_2(C')\geq 0$}{
Let $C\gets$ the first such cycle\\
$\Flag\gets \True$\\
}
}
\uIf{$\Flag$}{
Update $Q\gets Q\circ C$\\
Update $S\gets S\setminus C$\\
}
}
Update $Q\gets Q\circ S$\\
\Return{$Q$}
\end{algorithm}





==> d1d1_algorithm_bk.tex <==
\subsection{Algorithm for $\Dyck_1\odot \Dyck_1$}\label{subsec:d1d1_algo}

The bounded-paths property implies a straightforward algorithm to solve $\Dyck_1\odot \Dyck_1$ reachability.
Let $c$ be the counter bound of the bounded-paths lemma.
We  flatten the graph on one counter, by associating each node with all possible values of that counter.
This increases the graph size by a factor $c$, but reduces the interleaved Dyck reachability problem to standard Dyck reachability.
Hence, we can use the existing optimal algorithm for bidirected graphs~\cite{Chatterjee18}.
We present this algorithm in detail.


\Paragraph{Algorithm for $\Dyck_1\odot\Dyck_1$ reachability.}
Consider an input  interleaved bidirected Dyck graph $G=(V,E, \Alphabet=\Alphabet_1\DUnion\Alphabet_2)$ with $n$ nodes, and let $c=4\cdot n\cdot(n-1)+8\cdot n$.
We construct the bidirected Dyck graph $G'=(V', E', \Alphabet')$ as follows.
\begin{compactenum}
\item The node set of $G'$ is $V'=V\times (\{0\}\cup [c])$.
\item The edge set of $G'$ is such that, for every edge $(u,v,\gamma)\in E$ and $j\in \{0\}\cup [c]$, we have an edge $((u,j_1), (u,j_2), \delta)\in E'$, as follows.
\begin{compactenum}
\item If $\gamma\in \Alphabet_1\cup \{\epsilon\}$, then $j_2=j_1$ and $\delta=\gamma$.
\item If $\gamma\in \Open(\Alphabet_{2})$ and $j_1<c$, then $j_2=j_1+1$ and $\delta=\epsilon$.
\item If $\gamma\in \Close(\Alphabet_{2})$ and $j_1>0$, then $j_2=j_1-1$ and $\delta=\epsilon$.
\end{compactenum}
\end{compactenum}

Note that since $G$ is bidirected, $G'$ is also bidirected (that is, on the alphabet $\Alphabet_{1}$).
Afterwards, we use the algorithm from~\cite{Chatterjee18} to solve $\Dyck_1$-reachability on $G'$.
We return that two nodes $u,v\in V$ belong to the same reachability class in $G$ iff $(u,0), (v,0)$ belong to the same reachability class of $G'$.
We conclude with the correctness and complexity of the algorithm, which proves \cref{thm:d1d1_upper_bounds}.

\begin{proof}[Proof of \cref{thm:d1d1_upper_bounds}]
We start with the correctness.
For any path $P\colon u\Path v$ in $G$ with $\MaxCounter_1(P)\leq c$, there exists a path $P'\colon (u,0)\Path (v, \ell)$ in $G'$, such that $\ell=\Counter_1(P)$ and $\Counter_2(P)=\Counter_2(P')$.
By \cref{lem:d1d1bounded_paths}, if a node $v$ is $\Dyck_1\odot\Dyck_1$-reachable from a node $u$ in $G$, then there exists a witness path $P$ with $\MaxCounter_j(P)\leq c$ for each $j\in[2]$.
Thus there exists a corresponding path $P'\colon (u,0)\Path (v,0)$ in $G'$, which means that $(u,0)$ and $(v,0)$ are in the same reachability class of $G'$.
The correctness hence follows from the correctness of the algorithm of~\cite{Chatterjee18} for $\Dyck_1$-reachability.


We now turn our attention to the complexity.
By \cref{lem:d1d1bounded_paths}, the graph $G'$ has $O(n\cdot c)$ nodes.
By \cref{rem:bounded_degree}, the graph $G$ is sparse, which implies that $G'$ is also sparse, i.e., $G'$ has $O(n\cdot c)$ edges.
By~\cite{Chatterjee18}, solving $\Dyck_{1}$-reachability on $G'$ requires $O(n\cdot c\cdot \alpha (n))$ time.
The desired result follows.
\end{proof}





==> d1d1_bk.tex <==
\section{A Fast Algorithm for $D_1\odot D_1$}\label{sec:d1d1}

In this section we deal with the $D_1\odot D_1$, i.e., when both Dyck languages are over a unary alphabet.
%Note that in this case each stack behaves as a non-negative counter.
%To make this case explicit, we will speak about the value of counter $i\in[2]$ along a path, instead of the height of the corresponding stack.
%For each $i\in [2]$, we let $\Counter_i=\StackHeight_i(P)$ and $\MaxCounter_i(P)=\MaxStackHeight_i(P)$.
%Moreover, we define $\MinCounter_i(P)=\min_{P'} \Counter_i(P')$, where $P'$ ranges over prefixes of $P$.
%In words, $\MinCounter_i(P)$ is the smallest value of counter $i$ along $P$.


\Paragraph{Shallow paths.}
The key insight behind the algorithm of~\cite{Li2021} is that paths that serve as reachability witnesses exhibit a ``shallow-paths'' property, which states that wlog, along every witness path one of the two counters is linearly bounded.
We restate the property in the following lemma.
\begin{restatable}[Shallow Paths~\cite{Li2021}]{lemma}{lemd1d1shallowpaths}\label{lem:d1d1shallow_paths}
For any nodes $u,v\in V$ such that $v$ is $\Dyck_1\odot \Dyck_1$-reachable from $u$, 
there exists a path $P\colon u\DODOPath v$ such that
for every prefix $P'\in \Prefixes(P)$, we have $\Counter_i(P')\leq 6\cdot n$ for some $i\in [2]$.
\end{restatable}



\Paragraph{Bounded paths.}
The key insight behind our improvement is that we can assume that each counter is \emph{always} bounded by $O(n^2)$.
%while if the graph has no same-sign cycles, this bound reduces to $O(n)$ (i.e., from quadratic to linear).
The following lemma states this stronger ``bounded-paths'' property.
\begin{restatable}[Bounded Paths]{lemma}{lemd1d1boundedpaths}\label{lem:d1d1bounded_paths}
For any nodes $u,v\in V$ such that $v$ is $\Dyck_1\odot \Dyck_1$-reachable from $u$, 
there exists a witness path $P\colon u\DODOPath v$ such that $\MaxCounter_i(P)\leq 4\cdot n\cdot (n-1) + 8\cdot n$ for each $i\in[2]$.
%Moreover, if the input graph has no same-sign cycles, then there exists a witness path $P\colon u\Path v$ such that $\MaxCounter_i(P)\leq 8\cdot n$ for each $i\in[2]$.
\end{restatable}

\input{figures/counter_bound}

We remark that the $O(n^2)$ bound of \cref{lem:d1d1bounded_paths} is tight:
\cref{fig:counter_bound} shows a simple example where in every $P\colon u\DODOPath v$ path, each counter reaches $\Theta(n^2)$.
% (note, however, that the example has same-sign cycles).
This section is split in two parts.
First, we assume the bounded-paths property (i.e., \cref{lem:d1d1bounded_paths}),
and based on it, we present an algorithm to obtain \cref{thm:d1d1_upper_bounds}.
Afterwards we prove \cref{lem:d1d1bounded_paths}.





\input{d1d1_algorithm}
\input{d1d1_bounded_paths}



==> d1d1_bounded_paths_bk.tex <==
\subsection{Bounded Paths in $\Dyck_1\odot \Dyck_1$}\label{subsec:d1d1_bounded_paths}

Here we prove \cref{lem:d1d1bounded_paths}.
The section is somewhat technical and can be be skipped at first, as later sections do not depend on it.
We remark that our main goal is to show a quadratic upper-bound on each counter along a path that witnesses
 $\Dyck_1\odot \Dyck_1$ reachability.
As such, our proof aims at readability, without necessarily establishing the smallest constant factor in this bound.
Consider that we have a path $P\colon u\DODOPath v$.
The main steps of the proof are as follows.

\begin{compactenum}
\item\label{item:d1d1_outline1} First we establish that either we have a path $Q\colon u\DODOPath v$ in which every counter stays upper-bounded by $8\cdot n$,
or $u$ can reach a same-sign cycle $K_u$ with both counters upper-bounded by $9\cdot n+1$.
Note that in the former case the bound is within the bound of \cref{lem:d1d1bounded_paths} and we are done.
In the latter case, we proceed with the next step.
%Note that this step already proves the linear bound of \cref{lem:d1d1bounded_paths} when the input graph has no same-sign cycles.
\item\label{item:d1d1_outline2} Since $u$ can reach such a cycle $K_u$, we can construct a cyclic path $F_u\colon u\Path u$ in which both counters remain between $2\cdot n$ and $\gamma=2\cdot n\cdot (n-1)$, by traversing $K_u$ sufficiently many times.
\item\label{item:d1d1_outline3} Given the path $F_u$, we construct a path $W_u=F_u\circ Z$ from $u$ to $v$ such that both counters remain upper-bounded by $\gamma+8\cdot n$.
On the other hand, we have $\Counter_i(W_u)=\Counter_i(F_u)\geq 2\cdot n$,
and hence $W_u$ does not witness the reachability of $v$ from $u$.
Nevertheless, we next extend $W_u$ suitably to obtain a witness path.
\item\label{item:d1d1_outline4} Repeating the argument of \cref{item:d1d1_outline2} for $v$, we construct a path $F_v\colon v\Path v$ in which both counters remain between $2\cdot n$ and $\gamma$.
Finally we construct the path (see \cref{fig:all}) 
\[
T\colon F_u\circ Z\circ F_v\circ \ov{Z} \circ \ov{F}_u \circ Z \circ \ov{F}_v
\]
which witnesses the $\Dyck_1\odot \Dyck_1$-reachability of $v$ from $u$, and in which both counters remain bounded by $2\cdot \gamma + 8\cdot n$.
\end{compactenum}

\input{figures/all}

In the following we present steps 1-4 in detail.



\Paragraph{Step~1:~Path deflation.}
Consider a path $P\colon u\DPath{\Dyck_1\odot \Dyck_1} v$ such that $\MaxCounter_i(P)>  8\cdot n$ for some $i\in [2]$
(clearly, if no such path exists then the lemma follows trivially).
We assume wlog that $P$ satisfies the shallow-paths property (\cref{lem:d1d1shallow_paths}).
Let $P'$ be the shortest prefix of $P$ such that $\Counter_i(P')=8\cdot n+1$ for some $i\in [2]$.
Hence, $P$ must have an $i$-negative cycle after $P'$.
We let $C$ be the first such cycle, $P_C$ be the prefix of $P$ up to the point where $C$ starts, and $P_1$ be a prefix of $P_C\circ C$ in which counter $i$ attains its highest value.
Note that $|P'|\leq |P_1| <|P_C\circ C|$, since $C$ is $i$-negative and, by our choice of $P'$, counter $i$ is below $8\cdot n$ in every strict prefix of $P'$.
Moreover, the shallow-path lemma guarantees that counter $(3-i)$ stays below $6\cdot n$ between the end of $P'$ and the end of $C$.
We also let $P_2$ be the suffix of $P$ such that $P=P_1\circ P_2$.
\cref{fig:path_dec} illustrates these paths for $i=1$.

\input{figures/path_dec}

The first step towards the bounded-paths lemma is that of path deflation, illustrated in \cref{fig:path_deflation}.
The key idea is that, instead of traversing the whole of $P$, we stop in the prefix $P''$ of $P'$ where counter $i$ takes the value $6\cdot n$ for the last time until it reaches the value $8\cdot n+1$ by the end of $P'$.
As the counter goes from $6\cdot n$ in the end of $P''$ to $8\cdot n+1$ in the end of $P'$, we have to traverse a cycle $H$ in between that is $i$-positive.
Now assume that
(i)~$H$ is not $(3-i)$-positive, and
(ii)~$C$ is not $(3-i)$-negative.
Then we can deflate the counter $i$ as follows.
\begin{compactenum}
\item From the end of $P''$, we traverse $P$ all the way to the beginning of $C$, but we omit $H$.
\item We traverse $C$.
\item We return back to the end of $P''$ by following the reverse path of step~1.
\end{compactenum}
This detour guarantees that we arrive at the end of $P''$ with counter $i$ having decreased by an offset between $1$ and $n$ (in particular, by the value of the $i$-negative cycle $C$), while counter $(3-i)$ has not decreased.
At this point we proceed along $P$ as originally.
Our assumptions about the impact of cycles $H$ and $C$ on counter $(3-i)$ guarantee that the resulting path is valid (i.e., the counter does not drop below 0).
At the same time, the  counter $(3-i)$ has increased by at most $2\cdot n$, hence it stays bounded by $8\cdot n$.
Importantly, because we have proactively traversed $C$ which is $i$-negative, at the end of $P_1$, counter $i$ has strictly decreased compared to its initial value.
Once we have reached the cycle $C$, the two counters obtain the values they had in the original path after traversing $C$, and the path now extends as before all the way to $v$ (while skipping $C$).
%Overall, the value of counter $i$ has deflated at the end of $P_1$, where it reached its maximum value initially.
This observation is formally captured in the following lemma.


\input{figures/path_deflation}
\begin{restatable}{lemma}{lempathdeflation}\label{lem:path_deflation}
At least one of the following holds.
\begin{compactenum}
\item\label{item:d1d1_n_or_positive_cycle_item1}
There is a path $Q\colon u\DODOPath v$ where $Q=Q_1\circ Q_2$ such that
(i)~$\MaxCounter_i(Q_1)<\MaxCounter_i(P_1)$,
(ii)~$\MaxCounter_{(3-i)}(Q_1)\leq 8\cdot n$, and
(iii)~$|Q_2|<|P_2|$.
\item\label{item:d1d1_n_or_positive_cycle_item2}
$P$ has a same-sign cycle $K$ reachable from $u$ via a path $L$ such that
$\MaxCounter_{j}(L)\leq 9\cdot n+1$ for each $j\in [2]$.
\end{compactenum}
\end{restatable}


If $P$ has no same-sign cycle, we can apply \cref{item:d1d1_n_or_positive_cycle_item1} of  \cref{lem:path_deflation} to obtain another path $Q\colon u\DODOPath v$ in which counter $i$ is \emph{deflated} from its first local maximum above $8\cdot n$ to a strictly smaller value.
By repeated applications of \cref{lem:path_deflation}, we either arrive at a path that has a same-sign cycle, or obtain a path $u\DODOPath v$ in which both counters stay below $8\cdot n$.
We thus have the following lemma.

\begin{restatable}{lemma}{lemd1d1linearbound}\label{lem:d1d1_linear_bound}
At least one of the following holds.
\begin{compactenum}
\item\label{item:d1d1_linear} There exists a path $Q\colon u\DODOPath v$ with $\MaxCounter_{i}(Q)\leq 8\cdot n$ for each $i\in [2]$.
\item\label{item:d1d1_cycle} There exists same-sign cycle $K_u$ reachable from $u$ via a path $L_u$ such that
$\MaxCounter_{j}(L_u)\leq 9\cdot n+1$ for each $j\in [2]$.
\end{compactenum}
\end{restatable}

Note that \cref{item:d1d1_linear} of the lemma is within the bounds of \cref{lem:d1d1bounded_paths}.
The natural remaining question hence, is what happens in the case that $P$ has a same-sign cycle.
The key idea is now a form of path \emph{inflation}, where we traverse the same-sign cycle in the orientation that increases the value of both counters sufficiently, so that future applications of path deflation can take place without assumptions on the impact of cycles $H$ and $C$ on counter $(3-i)$.



\Paragraph{Step~2:~Path inflation.}
We now describe path inflation in detail.
Let $\gamma=2\cdot n\cdot (n-1)$.
Consider that there exists a cycle $K_u$ that is both $1$-positive and $2$-positive,
and that $K_u$ is reachable from $u$ via a path $L_u$ such that $\MaxCounter_{i}(L_u)\leq 9\cdot n+1$.
We let $\ell$ be the smallest integer $j$ such that $j\cdot \Counter_i(K_u)\geq 2\cdot n$  for each $i\in [2]$.
Hence $\ell$ gives us the smallest number of times he have to iterate $K_u$ in order to inflate each counter by at least $2\cdot n$.
We construct a cyclic path $F_u\colon L_u\circ K_u^{\ell}\circ \ov{L}_u$, where $K_u^{\ell}$ denotes $\ell$ iterations of $K_u$.
The following lemma is straightforward.

\begin{restatable}{lemma}{lempathinflation}\label{lem:path_inflation}
For each $i\in[2]$, we have 
(i)~$ 2\cdot n\leq\Counter_i(F_u)\leq \gamma$, and
(ii)~$\MaxCounter_i(F_u)\leq \gamma$,
where $\gamma=2\cdot n\cdot (n-1)$.
\end{restatable}

Conceptually, \cref{lem:path_inflation} states that if we can reach a same-sign cycle via a path in which each counter is bounded,
we can traverse the cycle in the positive orientation (i.e., the orientation that both counters increase) enough times to inflate each counter to a value at least $2\cdot n$, while both counters remain upper-bounded by $\gamma$.
Based on this observation, we revisit the path deflation idea of \cref{lem:path_deflation}, but this time assuming that both counters are lower-bounded by $2\cdot n$.
%To maintain the correspondence with the paths described in \cref{lem:path_deflation}, we use calligraphic symbols
%(e.g., path $P$ becomes path $\mathcal{P}$).

%\input{figures/path_deflation2}


\Paragraph{Step~3:~Deflating inflated paths.}
Consider the $u\Path v$ path $F_u\circ P$, where $F_u$ is the path defined in Step~2 and $P$ is the path defined in Step~1.
That is, we have $\MaxCounter_i(P)> 8\cdot n$ for some $i\in [2]$.
Consider again the cycles $H$ and $C$ in the path $P$ as defined in Step~1,
but without making any assumptions about the effect of cycles $H$ and $C$ on counter $(3-i)$.
We rearrange $P$ in the same way, namely:
\begin{compactenum}
\item From the end of $P''$, we traverse $P$ all the way to the beginning of $C$, by we omit $H$.
\item We traverse $C$.
\item We return back to the end of $P''$ by following the reverse path of step~1.
\end{compactenum}
Let $Z$ be the resulting path after the rearrangement of $P$.
The rearrangement guarantees that we arrive at $P''$ with counter $i$ having decreased in value by an offset between $1$ and $n$.
Moreover, the detour changes counter $(3-i)$ (either increase or decrease) by at most $2\cdot n$.
Although the counter can now become negative $Z$, it remains non-negative in the path $F_u\circ Z$.
By applying this process repeatedly until $\MaxCounter_i(P)< 8\cdot n$ for each $i\in [2]$,
we end up with a path $W_u\colon u\Path v$ of the form $W_u\colon F_u\circ Z$ in which both counters remain bounded by $\gamma+8\cdot n$.
This is formally stated in the following lemma.



\begin{restatable}{lemma}{lempathdeflation}\label{lem:path_deflation2}
For each $i\in[2]$, we have $\MaxCounter_i(W_u)\leq \gamma+8\cdot n$.
\end{restatable}

Note that the path $W_u$ does not witness the $\Dyck_1\odot \Dyck_1$ reachability of $v$ from $u$, as $\Counter_i(W_u)=\Counter_i(F_u)\geq 2\cdot n$ for each $n$.
Nevertheless, we can use $W_u$ to construct a reachability witness, as we show in the next and final step.



\Paragraph{Step~4:~Putting it all together.}
We are now ready to combine all the pieces of the proof of \cref{lem:d1d1bounded_paths}.
As we have argued in Step~3, we can construct a path $W_u\colon F_u\circ Z$, where $F_u\colon u\Path u$ such that $\MaxCounter_i(W_u)\leq \gamma+8\cdot n$.
Following the exact same process symmetrically for $v$ instead of $u$, we can also construct a path $W_v\colon F_v\circ \ov{Z}$, where $F_v\colon v\Path v$ is a cyclic path such that $\MaxCounter_i(W_v)\leq \gamma+8\cdot n$.
Then, we construct the path $T\colon u \DODOPath v$ as 
\[
T\colon F_u\circ Z\circ F_v\circ \ov{Z} \circ \ov{F}_u \circ Z \circ \ov{F}_v
\]
\cref{fig:all} illustrates the path $T$ and the upper-bounds of each counter along various segments of $T$.
In particular, the maximum value of each counter is upper-bounded by $2\cdot \gamma + 8\cdot n$, reached in the prefix 
$F_u\circ Z\circ F_v$.
Hence, \cref{lem:d1d1bounded_paths} follows.






==> dkd1_bounded_counters.tex <==
\subsection{The Case of Bounded Counters}\label{subsec:dkd1_bounded_counters}


\input{figures/ov}

==> dkd1_lower_bound.tex <==
\subsection{$\Dyck_k\odot \Dyck_1$ Reachability Lower Bound}\label{subsec:dkd1_lower_bound}

Here we present the $\NP$-hardness of $\Dyck_k\odot \Dyck_1$ reachability.
The key observation is that, due to the presence of the stack,
the counter can become exponentially large along a path that witnesses reachability.
This way, the counter can encode an exponentially large search space of $\NP$-hard problems.

\Paragraph{Reduction.}
We show \cref{thm:dkd1_np_hard} by establishing a reduction from the Subset Sum problem.
The input to Subset Sum is a pair $(X,S)$, where $X=\{ x_1, \dots, x_n \}$ is a multi-set of positive natural numbers,
and $S$ is also a positive natural number, such that $x_i\leq S$ for each $i\in [n]$.
The task to find a subset of indices $A\subseteq [n]$ such that $\sum_{i\in A} x_{i}=S$.
We let $j_{\max}$ be the smallest integer such that $S\leq 2^{j_{\max}}-1$, i.e., $j_{\max}$ is the most significant bit in the binary representation of $2\cdot S$.
We construct an interleaved and bidirected Dyck graph $G=(V,E,\Alphabet=\Alphabet_k\DUnion\{+1,-1 \})$ such that for two distinguished nodes $u,v\in V$ we have $u\DKDOPath v$ iff the Subset Sum instance is positive.



\Paragraph{Intuition.}
In high level, we construct a graph that has a pipeline form, and the different segments along the way correspond to gadgets that represent the various $x_i$'s.
A path opens a parenthesis of $\Alphabet_k$ when it chooses the respective $x_i$ in the solution of subset sum, while it uses the counter to keep track of the running sum of all $x_i$.
In more detail, our reduction is based on two gadgets, illustrated in \cref{fig:np_hard_gadgets}.
\begin{compactenum}
\item For every $\ell\in [j_{\max}]$, we have two \emph{power gadgets} $G_{\ell}^+$ and $G_{\ell}^-$  .
Each power gadget is a graph with an entry node $p$ and an exit node $q$, with the property that $q$ is $\Dyck_k$-reachable from $p$ in $G_{\ell}^{+}\Project \Alphabet_1$ and $G_{\ell}^{-}\Project \Alphabet_1$.
That is, in both graphs $G_{\ell}^{+}$ and $G_{\ell}^{-}$, we have a valid path $P\colon p\Path q$ that starts and ends with an empty stack.
Moreover, every such path in $G_{\ell}^{+}$ (resp., $G_{\ell}^{-}$) increases (resp., decreases) the counter by $2^\ell$.
\item For every positive integer $x$ in $X$, we have a \emph{counter gadget} $H^+_{x}$ that increases the counter value by $x$.
We construct $H^+_{x}$ by serially connecting the power gadgets $G_{j_1}^+, G_{j_2}^+, \dots, G_{j_l}^+$,
where the $j_i$ are chosen such that $x=\sum_i 2^{j_i}$.
Similarly we have a counter gadget $H^-_{-2\cdot S}$.
\end{compactenum}
We combine the counter gadgets to construct the graph $G$, consisting of two subgraphs (see \cref{fig:np_hard}).
The first sub-graph is based on a sequence of nodes $u_1,\dots, u_n$,
while the second sub-graph is based on  a sequence of nodes $v_n,\dots v_1, v$.
Each node $u_i$ can reach node $u_{i+1}$ in two paths.
The first path goes through the counter gadget $H_{x_i}$, which increments the counter by $x_i$, and corresponds to choosing $x_i$ in our solution to Subset Sum.
The other path is just a single edge, which corresponds to not choosing $x_i$ in our solution.
To avoid cycles formed by these two paths due to bidirectedness, the first path also pushes $\delta_1$ on the stack, while the second path pushes $\delta_0$.
The process repeats symmetrically on the second part of the graph along the nodes $v_n,\dots, v_1$, only that now we pop the corresponding symbols from the stack in reverse order.
%The process continues until node $v_1$, which is connected to the gadget $H_{-2\cdot S}$.
This way, any path from $P\colon u_1\DKDOPath v$ will take the outgoing edge labeled with $\delta_1$ from each $u_i$, iff it takes the outgoing edge labeled with $\ov{\delta}_1$ from $v_i$. 
By choosing these edges that correspond to a solution for Subset Sum, the counter will equal $2\cdot S$ when $P$ reaches node $v_1$, while the stack will be empty.
At that point $P$ will traverse the counter gadget $H_{-2\cdot S}$, to reach $v$,
which verifies the solution set to subset sum.

\input{figures/np_hard_gadgets}



\Paragraph{Formal construction.}
We now present the formal construction.
We first define the two gadgets and then connect the gadgets together to obtain the interleaved Dyck graph $G=(V,E,\Alphabet)$. 



\SubParagraph{The power gadgets.}
Let $\Alphabet_{\gamma}=\{ \gamma_0, \gamma_1, \ov{\gamma}_0, \ov{\gamma}_1 \}$ be a Dyck alphabet.
Given some natural number $\ell$, we construct two interleaved Dyck graphs $G_{\ell}^+=(V_{\ell}^+, E_{\ell}^+,\Alphabet_{\gamma} \DUnion \{ +1, -1\})$
and $G_{\ell}^-=(V_{\ell}^-, E_{\ell}^-,\Alphabet_{\gamma} \DUnion \{ +1, -1\})$.
Both graphs have a single edge that manipulates the counter. 
The graphs are identical, with the difference that $G_{\ell}^+$ increments the counter along the edge while $G_{\ell}^-$ decrements the counter.
Hence it suffices to define $G_{\ell}^+$.
The node set is $V_{\ell}^+= \{p,q\} \cup \bigcup_{i\in[\ell]}\{ a_i, b_i, c_i \}$, and we have the following labeled edges.
\begin{compactenum}
\item For every $i \in [\ell]$, we have $c_{i}\DTo{\ov{\gamma}_0}b_{i}$ and $b_{i}\DTo{\gamma_1}a_i$.
\item For every $i\in [\ell-1]$, we have $a_{i+1}\DTo{\gamma_0} a_i$ and $c_i\DTo{\ov{\gamma}_1}c_{i+1}$.
We also have $p\DTo{\gamma_0} a_{\ell}$ and $c_{\ell}\DTo{\ov{\gamma}_0} q$.
\item We have $a_1\DTo{+1}c_1$ (while we have $a_1\DTo{-1}c_1$ in $G_{\ell}^-$).
\end{compactenum}
We call $p$ and $q$ and entry node and exit node of $G_{\ell}^+$, respectively.
See \cref{fig:np_hard_gadgets} for an illustration.

\input{figures/np_hard}


\SubParagraph{The counter gadgets.}
For every $i\in [n]$, consider the integer $x_i$.
We construct a counter gadget $H_{x_i}$, as follows.
Let $j_1,\dots, j_{\ell}$ be natural numbers such that $x_i=\sum_{l\in [\ell]}2^{j_l}$.
We connect serially the power gadgets $G^+_{j_l}$, i.e., we connect the exit node of gadget $G^+_{j_l}$ to the entry node of gadget $G^+_{j_{l+1}}$.
The entry node (resp., exit node) of $H_{x_i}$ is the entry node (resp., exit node) of $G^+_{j_1}$ (resp., $G^+_{j_{\ell}}$).
%We similarly construct a counter gadget $H_{-x_i}$ by connecting the power gadgets $G^-_{j_l}$.
%Hence, traversing the gadget $H_{x_i}$ (resp., $H_{-x_i})$, increases (resp., decreases) the counter by $x_i$.
Finally, we construct a similar gadget $H_{-2\cdot S}$, by connecting the appropriate power gadgets $G^-_{j_i}$ in the binary representation of $2\cdot S=\sum_{l\in [\ell]}2^{j_l}$.




\SubParagraph{Putting it all together.}
To complete the construction, we now describe how to construct the $\Dyck_k\odot \Dyck_1$ Dyck graph $G=(V,E,\Alphabet)$ by connecting the gadget graphs together.
The alphabet is $\Alphabet= \Alphabet_{\gamma}\cup \Alphabet_{\delta}$, where
$\Alphabet_{\gamma}$ is the alphabet of the counter gadgets, and
 $\Alphabet_{\delta}=\{ \delta_0, \delta_1, \ov{\delta}_0, \ov{\delta}_1 \}$.
The graph consists of the following nodes and edges (see \cref{fig:np_hard}).
\begin{compactenum}
\item We have nodes $u_1,\dots, u_n, d, v_1,\dots v_n, v$.
\item For every $i\in[n]$ we have two copies of the counter gadget $H_{x_i}$. We also have one counter gadget $H_{-2\cdot S}$.

\item For every $i\in[n]$, we have an edge $u_i\DTo{\delta_1} p^1_i$, where $p_i^1$ is the entry node of the first copy of the counter gadget $H_{x_i}$.

\item For every $i\in[n-1]$, we have an edge $u_i\DTo{\delta_0}u_{i+1}$, and an edge $q_i^1\DTo{}u_{i+1}$, where $q_i^1$ is the exit node of the first copy of the counter gadget $H_{x_i}$.

\item We have edges $u_n\DTo{\delta_0}d$, $c_n^1\DTo{}d$, $d\DTo{\ov{\delta}_0}v_n$ and $d\DTo{\ov{\delta}_1} a_n^2$,
where $c_n^1$ is the exit node of the first copy of the counter gadget $H_{x_n}$, and $a_n^2$ is the entry node of the second copy of the counter gadget $H_{x_n}$.

\item For every $i\in[n]$, we have an edge $c_i^2\DTo{} v_i$, where $c_i^2$ is the exit node of the second copy of the counter gadget $H_{x_i}$.


\item For every $i\in[n-1]$, we have an edge $v_{i+1}\DTo{\ov{\delta}_0}v_{i}$, and an edge $v_{i+1}\DTo{\ov{\delta}_1}a_i^2$, where $a_i^2$ is the entry node of the second copy of the counter gadget $H_{x_i}$.


\item Finally, we have an edge $v_1\DTo{}a_{2\cdot S}$ and $c_{2\cdot S}\DTo{}v$, where $a_{2\cdot S}$ and $c_{2\cdot S}$ are the entry and exit nodes, respectively, of the counter gadget $H_{-2\cdot S}$.
\end{compactenum}





\Paragraph{Correctness.}
We now turn our attention to the correctness of the construction, and argue that 
$v$ is $\Dyck_k\odot \Dyck_1$-reachable from $u_1$ iff there is a set $A\subseteq [n]$ such that $\sum_{i\in A} x_i=S$.
The first lemma concerns the behavior of the power gadgets.
It states that any path from the entry node to the exit node of a power gadget increases/decreases the counter value by the corresponding power of $2$.


\begin{restatable}{lemma}{lemdkdonepowergadget}\label{lem:dkd1_power_gadget}
For every power gadget $G_{\ell}^+$ (resp., $G_{\ell}^-$),
for every valid path $P\colon p\Path q$ with $\Stack(P)=\epsilon$, where $p$ and $q$ are the entry and exit node of $G_{\ell}^+$ (resp., $G_{\ell}^-$),
we have $\Counter_1(P)=2^{\ell}$ (resp., $\Counter_1(P)=-2^{\ell}$).
\end{restatable}


Using \cref{lem:dkd1_power_gadget}, it is straightforward to prove that the counter gadgets have the desired effect on the counter, as stated in the following lemma.

\begin{restatable}{lemma}{lemdkdonecountergadget}\label{lem:dkd1_counter_gadget}
For every counter gadget $H_{x_i}$ ( resp., for the counter gadget $H_{-2\cdot S}$),
for every valid path $P$ from the entry node to the exit node of $H_{x_i}$ (resp., $H_{-2\cdot S}$),
if $\Stack(P)=\epsilon$ then $\Counter(P)=x_i$ (resp., $\Counter(P)=-2\cdot S$).
\end{restatable}


Using \cref{lem:dkd1_counter_gadget}, we can now prove the correctness of the construction.
The key insight is that any irreducible path $P\colon u_1\Path v$ never traverses an edge in both directions.
As $P$ goes along the nodes $u_i$, it chooses the outgoing edges labeled with $\delta_1$ to traverse the corresponding counter gadget $H_{x_i}$, which increases the counter by $x_i$.
This corresponds to choosing $x_i$ in the solution to the Subset Sum problem.
On the other hand, traversing an edge labeled with $\delta_0$ does not modify the counter, and corresponds to not choosing $x_i$ in the solution to the Subset Sum problem.
When the path reaches node $d$, the solution to the Subset Sum problem is encoded in the stack of the path, while the counter holds the corresponding value (which is equal to $S$).
In order to pop the elements of the stack, $P$ is forced to choose the mirrored outgoing edges when traversing the nodes $v_i$.
Hence $P$ has to traverse the same counter gadgets along $v_i$ as it did along $u_i$. 
This has the effect that the stack is emptied when $P$ reaches $v_1$, but the counter has reached the value $2\cdot S$.
To verify that the solution is correct, $P$ is finally forced to traverse the counter gadget $H_{-2\cdot S}$, and reach $v$ with the counter being $0$.
We thus have the following lemma.


\begin{restatable}{lemma}{lemdkdonecorrectness}\label{lem:dkd1_correctness}
We have $u_1\DKDOPath v$ iff $(X,S)$ has a positive answer.
\end{restatable}


We are now ready to prove \cref{thm:dkd1_np_hard}.


\begin{proof}[Proof of \cref{thm:dkd1_np_hard}.]

\cref{lem:dkd1_correctness} establishes the correctness of the reduction, so here we turn our attention to the complexity (i.e., we argue that the reduction is done in $\PTime$).
As we have linearly many gadgets and nodes $u_i$ and $v_i$, it suffices to argue that the size of the largest counter gadget (i.e, gadget $H_{-2\cdot S}$) is polynomial in the size of the input.
Indeed, observe that the $\ell$-th non-zero bit of $-2\cdot S$ is encoded by a power gadget $G^{-}_{\ell}$ which contains only $O(\ell)$ nodes.
Hence the size of $H_{-2\cdot S}$ is quadratic in the bit-length of the encoding of $S$.
Thus the size of $G$ is polynomial in the size of $(X,S)$, while the construction of $G$ is easily carried out in time linear in the size of $G$.
The desired result follows.
\end{proof}


==> dkd1_reduction.tex <==
\section{From General to Bidirected Reachability}\label{sec:dkd1_reduction}


\input{figures/reduction_gadgets}
\input{figures/reduction}

\Paragraph{Construction.}
Consider a graph $G=(V,E,\Alphabet=\Alphabet \DUnion \{-1,0,1 \} )$ and two nodes $u,v\in V$.
We construct a graph $G'=(V', E', \Alphabet'=\Alphabet'\DUnion\{-1,0,1 \})$ with two nodes $s,t\in V'$ such that
$s\DKDOPath t$ in $G'$ iff $u\DKDOPath v$ in $G$.

\SubParagraph{The alphabet $\Alphabet'$.}
We construct the alphabet $\Alphabet'$
\[
\Alphabet'=\Alphabet \cup E \cup \ov{E}
\]
8

==> dkdk_bk.tex <==
\section{Undecidability of $D_k\odot D_k$}\label{sec:dkdk}

Finally, in this section we study the general $D_k\odot D_k$ reachability on bidirected graphs, and show that the problem is undecidable (\cref{thm:dkdk_undecidable}).
Our reduction is from $D_k\odot D_k$ reachability on non-bidirected graphs, which is known to be undecidable~\cite{Reps00}.

\Paragraph{Reduction.}
Consider a graph $G=(V,E,\Alphabet)$ where $\Alphabet=\Alphabet_1\DUnion\Alphabet_2$,
and the problem of  $D_k\odot D_k$ reachability wrt the alphabets $\Alphabet_1$ and $\Alphabet_2$ on two nodes $u$ and $v$ of $G$.
We construct a graph $G'=(V', E', \Alphabet')$ where $V\subset V'$ and $\Alphabet'=\Alphabet'_1\DUnion\Alphabet'_2$,
and such that a node $t\in V'$ is $D_k\odot D_k$-reachable from node $s\in V'$, wrt the alphabets $\Alphabet'_1$ and $\Alphabet'_2$, iff $v$ is reachable from $u$ in $G$.
To keep the exposition simple, the alphabet $\Alphabet'$ depends on $G$.
Standard constructions can turn $\Alphabet'$ to constant, though this comes at the expense of increasing the graph size by a logarithmic factor (see, e.g.,~\cite{Chistikov21}).
Since here we show undecidability, this increase is not a concern.


\input{figures/undecidability_gadgets}



\Paragraph{Intuitive description.}
We start with the intuition behind the reduction, while we refer to \cref{fig:undecidability_gadgets} for relevant illustrations.
Given $G$ and nodes $u$ and $v$, we will construct $G'$ such that there is a path $P\colon u\Path v$ in $G$
iff there exists a path $P'\colon s\Path t$ in $G'$, as follows.
Initially, the path $P'$ ``guesses'' the path $P$ edge-by-edge in reverse order, while it
(i)~pushes every guess in the first stack, and
(ii)~uses the second stack to simulates the behavior of the second stack along $P$ in $G$ (in reverse), mirrored under the parenthesis complementation operator $\ov{\gamma}$
(i.e., if the edge in $G$ pushes $\gamma$, the simulating edge will pop $\gamma$).
Note that complementing the letters as found in the reverse order of $P$, in fact simulates the second stack in the forward order of $P$.

After this part is done, the second stack is empty, while the first stack contains the sequence of edges of $P$ in top-down order (i.e., the first edge of $P$ is at the top of the stack).
At this point, $P'$ will traverse the remaining of the graph $G'$ and verify that the path $P$ stored in first stack is a valid path of $G$.
As a preliminary step, $P'$ is forced to push two special symbols $\nu_1$ and $\nu_2$, one in each stack, as it takes a transition from $s$ to $u$.
This is a simple trick to deal with bidirectedness, in the sense that, if in the future $P'$ decides to come back to $s$ and alter the guessed path, it can only do so by popping $\nu_1$ and $\nu_2$ from their respective stacks.
This will imply that the second stack is empty and the first stack contains a suffix of the guessed $P$, and thus $P'$ is reducible.
%Thus, whatever modifications $P'$ makes on its guess for $P$ could already be made in the first step.

In order to verify the guess of $P'$, the graph $G'$ is constructed as follows (see \cref{fig:undecidability_gadgets}).
For every edge $e$ of $G$, we have a small gadget graph $G_e$ over five nodes $a,b,c,d,f$.
We have an edge $(a,b)$ that pushes in the second stack a special letter $\mu$.
Then we have several looping paths in $b$; the label of each path is such that it transfers a single letter from the first stack to the second stack (but not the letters corresponding to the guessed edges $e$). 
The edge $(c,d)$ is labeled with $\ov{e}$.
Using the self-loop in $b$, the path $P'$ can temporarily flush all its contents up to the top-most guessed edge (i.e., the  guessed edge that has not been traversed yet), and then transition to $c$, provided that the top-most guessed edge $e$ can be matched by $\ov{e}$.
Node $c$ has looping paths similar to $b$, that can now be traversed backwards and restore the first stack to its initial state, minus the matched edge symbol $e$.
Next, we have an edge $(c,d)$ labeled with $\ov{\mu}$, which ensures that the looping on $c$ restores the whole of the first stack, and the second stack becomes empty again.
Finally, we have an edge $(d,f)$ which carries the label $\Label(e)$, if $\Label(e)$ belongs to the first alphabet, otherwise the edge has an $\epsilon$ label (as the second stack of $G$ has already been simulated in the first step while self-looping on $s$).

The final part of the construction is having a path from $v$ to a distinguished node $t$ that pops the elements $\nu_1$ and $\nu_2$ from their respective stacks.
Hence, $s$ reaches $t$ in $G'$ iff $u$ reaches $v$ in $G$.

The key idea in the above description is that while self-looping over $s$, the path $P'$ can only guess the edges of $P$ in the direction they appear in $G$.
Although $P'$ can traverse edges backwards in $G'$,
this will generally result in pushing more edge symbols $e_1,\dots, e_{\ell}$ on the first stack.
Because of the letters $\nu_1$ and $\nu_2$, the only way to pop these symbols from the stack is for $P'$ to reverse the sub-path that added these symbols, which makes $P'$ reducible.

\cref{fig:undecidability} illustrates the above intuition on a small example.

\input{figures/undecidability}

\Paragraph{Construction.}
We now proceed with the formal construction.
We assume wlog that the reachability problem on $G$ is wrt to two nodes $u,v\in V$ where $s$ has no incoming edges and $t$ has no outgoing edges.
For ease of presentation, we specify some parts of $G'$ as paths, meaning unique sequences of labeled edges, without explicit reference to all the nodes and edges in the path.
We begin with the alphabets
\[
\Alphabet'_1 = \Alphabet_1 \cup \{\nu_1, \ov{\nu}_1 \} \cup \bigcup_{e\in E}\{ e, \ov{e} \} \qquad\qquad
\Alphabet'_2 = \Alphabet_2\cup \{\nu_2, \ov{\nu}_2, \mu, \ov{\mu} \} \cup \{\wh{\nu}_1, \ov{\wh{\nu}}_1 \} \cup \wh{\Alphabet}_1
\]
where $\wh{\Alphabet}_1$ contains a marked version of each element of $\Alphabet_1$ (so that $\Alphabet'_1$ and $\Alphabet'_2$ are disjoint).
Let $\Alphabet' = \Alphabet'_1\DUnion \Alphabet'_2$.
We first define a gadget graph $G_e=(V_e, E_e, \Alphabet')$ for every edge $e=(x,y,\gamma)\in E$, as follows.
\begin{compactenum}
\item $V_e=\{a,b,c,d,f\}$ is a set of five nodes, unique for the edge $e$.
\item We have edges $(a, b, \mu), (b,c,\ov{e}), (c,d,\ov{\mu})\in E_e$.
\item We have an edge $(c,d,\delta)\in E_e$, where $\delta=\gamma$ if $\gamma\in \Alphabet_1$ and $\delta=\epsilon$ otherwise.
\item For every opening parenthesis symbol $\kappa\in \{ \nu_1 \}\cup \Alphabet_1$, we have two cyclic paths $C_{\kappa}^b\colon b\Path b$ and $C_{\kappa}^c\colon c\Path c$ with label $\Label(C_{\kappa}^b)=\Label(C_{\kappa}^c)=\ov{\kappa} \wh{\kappa}$.
\end{compactenum}

We now proceed with the construction of $G'$.
We have $V\subset V'$, while $V'$ contains some additional nodes and edges, defined by the following paths.
For every edge $(x,y,\gamma)\in E$, we construct a cyclic path $C_e\colon s\Path s$
with $\Label(C_e)=e \delta$, where $\delta=\ov{\gamma}$ if $\gamma\in \Alphabet_2$ and $\delta=\epsilon$ otherwise.
We also construct a path $P_{s}\colon s\Path u$ with $\Label(P_{s})=\nu_1 \nu_2$.
For every edge $e=(x,y,\gamma)\in E$, we have two edges $(x,y', \epsilon), (x', y, \epsilon)\in E'$,
where$y'$ and $x'$ are the $a$-node and $f-$node of $G_e$, respectively.
Finally, we have a path $P_v\colon v\Path t$, where $t$ is a fresh node, with $\Label(P_v)=\ov{\nu}_2\ov{\nu}_1$.



\Paragraph{Correctness.}

\begin{restatable}{lemma}{lemdkdkcompleteness}\label{lem:dkdk_completeness}

\end{restatable}

\begin{restatable}{lemma}{lemdkdksoundness}\label{lem:dkdk_soundness}

\end{restatable}


\begin{proof}[Proof of \cref{thm:dkdk_undecidable}]
The proof follows directly from \cref{lem:dkdk_completeness} and \cref{lem:dkdk_soundness}.
\end{proof}

==> introduction-d38043.tex <==
\section{Introduction}\label{sec:intro}

Static analyses are one of the most common approaches to program analysis.
They offer tunable approximations to program behavior, by representing the set of possible program executions in the semantics of a simpler model (e.g., a graph, or a set of constraints) that is amenable to efficient analysis.
Although the model typically over-approximates program behavior, and may thus contain unrealizable executions,
it can be used to make sound conclusions of correctness, and even raise warnings of potential erroneous behavior.
In essence, this approach casts the semantic question of program correctness to an algorithmic question about the model (e.g., ``determine the existence of a path in a graph'', or ``find the least fixpoint to a system of constraints'').

\Paragraph{Dyck reachability.}
The standard formalism of a plethora of static analyses is via language graph reachability~\cite{Reps97}.
Informally the nodes of a graph represent various program segments (e.g., variables), 
while edges capture relationships between those segments, such as program flow or data dependencies.
In order to refine such relationships, the edges are annotated with letters of some alphabet.
This formalism reduces the analysis question to a reachability question between nodes in the graph,
as witnessed by paths whose labels along the edges produce a string that belongs to a language $\Language$.
Although $\Language$ varies per application, it is almost always a context-free/Dyck language,
yielding the problem commonly known as \emph{CFL/Dyck reachability}.

The Dyck reachability problem (denoted $\Dyck_k$) has applications to a very wide range of static analyses,
such as interprocedural data-flow analysis~\cite{Reps95}, slicing~\cite{Reps94}, 
shape analysis~\cite{Reps1995b}, impact analysis~\cite{Arnold96}, type-based flow analysis~\cite{Rehof01}, taint analysis~\cite{Huang2015},
data-dependence analysis~\cite{Tang2017},
alias/points-to analysis~\cite{Lhotak06,Zheng2008,Xu09}, and many others.
In practice, widely-used large-scale analysis tools, such as Wala~\cite{Wala} and Soot~\cite{Bodden12}, 
equip Dyck-reachability techniques to perform the analysis.
In all such cases, the balanced-parenthesis property of Dyck languages is ideal for expressing sensitivity of the analysis
in matching calling contexts, matching field accesses of composite objects, matching pointer references and dereferences etc.
This sensitivity improves precision in the obtained results and drastically reduces false positives.

\input{figures/example}

\Paragraph{Interleaved Dyck reachability and variants.}
When two types of sensitivity are in place simultaneously,
the underlying graph problem is lifted to \emph{interleaved} Dyck reachability over two Dyck languages (denoted $\Dyck_k\odot \Dyck_k$).
Intuitively, each language acts independently over its own alphabet to ensure sensitivity in one aspect (e.g., context vs field sensitivity).
This time, a path is accepted as a reachability witness iff the produced string wrt to each alphabet belongs to the respective language (see \cref{fig:example} for an illustration).
Unfortunately, interleaved Dyck reachability is well-known to be undecidable~\cite{Reps00}.
Nevertheless, the importance of the problem has lead to the development of various approximations that often work well in practice.
We refer to \cref{sec:related_work} for relevant literature in this area.

When a Dyck language is over a single parenthesis, the underlying stack acts as a counter.
This gives rise to variants of interleaved Dyck reachability, depending on whether one ($\Dyck_k\odot \Dyck_1$) or both ($\Dyck_1\odot \Dyck_1$) languages are over a single parenthesis.
Although these are less expressive models, they have rich modeling power and computational appeal.
For a $\Dyck_k\odot \Dyck_1$  example, $\Dyck_1$ can express that a queue is dequeued as many times as it is enqueued, and in the right order,
while $\Dyck_k$ is used as before to make the analysis context sensitive.
Similarly, $\Dyck_1\odot \Dyck_1$ can be used to identify an execution in which the program properly uses two interleaved but independent reentrant locks.


\Paragraph{Bidirected graphs.}
A Dyck graph is bidirected if every edge is present in both directions, and the two mirrored edges have complementary labels.
That is, $a\DTo{}b$ opens a parenthesis iff $b\DTo{}a$ closes the same parenthesis.
Bidirectedness turns reachability into an equivalence relation, much like the case of plain undirected graphs.
From a semantics perspective, bidirectedness is a standard approach to handle mutable heap data~\cite{Sridharan2006,Lu2019,Zhang2017}
-- though it can sometimes be relaxed for read-only accesses~\cite{Milanova2020},
and the de-facto formulation of demand-driven points-to analyses~\cite{Sridharan2005,Zheng2008,Shang2012,Yan11}.
Bidiretedness is also used for CFL-reachability formulations of pointer analysis~\cite{Reps97},
and has also been used for simplifying the input graph~\cite{Li2020}.
Thus in all these cases, the analysis yields the problem of \emph{interleaved bidirected Dyck reachability}.



\Paragraph{Open questions.}
Given the many applications of interleaved bidirected Dyck reachability, 
it is surprising that very little has been known about its decidability and complexity.
This gap is even more pronounced if contrasted to the rich literature on the complexity of Dyck reachability (see \cref{sec:related_work}).
The recent work of~\cite{Li2021} makes an important step in this direction, by proving an upper bound of $O(n^7)$ for $\Dyck_1\odot \Dyck_1$, and also showing  that the $\Dyck_k\odot \Dyck_k$ case is at least $\NP$-hard.
However, most of the fundamental questions remain unanswered, such as the following.
\begin{compactenum}
\item Although the $O(n^7)$ bound is polynomial, it remains prohibitively large.
Is there a faster algorithm, e.g., one that operates in quadratic/cubic time that is common in static analyses?
\item What is the decidability and complexity for $\Dyck_k\odot \Dyck_1$?
As $\Dyck_k\odot \Dyck_1$ is more expressive than $\Dyck_1\odot \Dyck_1$,
it leads to better precision in static analyses, and thus it is very well motivated.
Moreover, the non-bidirected case is also known as pushdown vector addition systems, 
where the decidability of reachability has been open (see \cref{sec:related_work}).
Is bidirectedness sufficient to show decidability? And if so, does it also make the problem tractable?
\item Given the undecidability of $\Dyck_k\odot \Dyck_k$ on general graphs,
does bidirectedness make the problem decidable?

\end{compactenum}

This work delivers several new results on the decidability and complexity of all variants of interleaved bidirected Dyck reachability, and paints the rich landscape of the problem.



\input{contributions}


%\input{related_work}

==> summary.tex <==
\section{Summary of Main Results}\label{sec:summary}

In this section we state formally the main theoretical results of this paper, and put them in context with regards to existing literature.
We consider as input a bidirected interleaved Dyck graph $G$ with $n$ nodes.

\Paragraph{Bidirected $\Dyck_1\odot \Dyck_1$ reachability.}
We start with the case of bidirected $\Dyck_1\odot \Dyck_1$ reachability.
The non-bidirected case falls into the class of vector addition systems with states.
In two dimensions, the problem is known to be in $\NL$ (and thus in $\PTime$)~\cite{Englert2016}.
The recent work of~\cite{Li2021} established an $O(n^7)$ bound for the bidirected case.
As our first theorem shows, the problem admits a must faster solution, namely, in essentially cubic time.

\smallskip
\begin{restatable}{theorem}{thmd1d1cubicupperbound}\label{thm:d1d1_upper_bounds}
Bidirected $\Dyck_1\odot \Dyck_1$ reachability can be computed in $O(n^3\cdot \alpha(n))$ time, where $\alpha(n)$ is the inverse Ackermann function.
%Moreover, the problem can be solved in $O(n^2\cdot \alpha(n))$ time over graphs with no same-sign cycles.
\end{restatable}

We obtain \cref{thm:d1d1_upper_bounds} by proving a boundedness property on paths witnessing reachability.
In particular, we show that wlog, along every such path \emph{both} counters remain quadratically bounded.
This strengthens the shallow-path property of~\cite{Li2021} which states that at any time \emph{one of the two counters} is bounded (though the bound is linear).

We next turn our attention to more expressive variants of interleaved Dyck reachability.

\Paragraph{Bidirected $\Dyck_k\odot \Dyck_1$ reachability.}
Here we address bidirected $\Dyck_k\odot \Dyck_1$ reachability.
The non-bidirected case is also known as pushdown vector addition systems in one dimension~\cite{Leroux2015},
for which the decidability of reachability is open.
Here we first show that bidirectedness suffices to make the problem decidable.

\smallskip
\begin{restatable}{theorem}{}\label{thm:dkd1_decidable}
Bidirected $\Dyck_k\odot \Dyck_1$ reachability is decidable.
\end{restatable}

The next natural question is whether bidirectedness, on top of decidability, further makes the problem tractable.
Our next theorem answers this question in negative.

\smallskip
\begin{restatable}{theorem}{thmdkd1nphard}\label{thm:dkd1_np_hard}
Bidirected $\Dyck_k\odot \Dyck_1$ reachability is $\NPH$.
\end{restatable}



Given the hardness of \cref{thm:dkd1_np_hard}, we next focus on the problem under a form of witness bounding,
which is a standard technique for efficient static analyses.
%~\cite{Xu2010,Chatterjee2017,Mathiasen2021}. 
In particular, we consider the case where reachability is witnessed by paths on which the counter stays linearly bounded
(though the stack has no restrictions).
We establish the following theorem.


\smallskip
\begin{restatable}{theorem}{thmdkd1quadraticupperbound}\label{thm:dkd1_quadratic_upper_bound}
Bidirected $\Dyck_k\odot \Dyck_1$ reachability with $O(n)$-bounded counters can be computed in $O(n^2\cdot \alpha(n))$ time, where $\alpha(n)$ is the inverse Ackermann function.
\end{restatable}

Hence, in contrast to the hardness of the general problem (\cref{thm:dkd1_np_hard}), restricting to a linear bound on the counter makes the problem efficiently solvable.
The next natural question is whether this restrictive setting admits even faster algorithms, e.g., can the problem be solved in $O(n)$ time?
We answer this question in negative.

\smallskip
\begin{restatable}{theorem}{thmdkd1quadraticupperbound}\label{thm:dkd1_quadratic_lower_bound}
For any fixed $\epsilon>0$,
bidirected $\Dyck_k\odot \Dyck_1$ reachability with $O(n)$-bounded counters cannot be solved in $O(n^{2-\epsilon})$ time under $\OV$.
\end{restatable}
Orthogonal Vectors ($\OV$) is a well-studied problem with a long-standing quadratic worst-case upper bound.
The corresponding hypothesis states that there is no sub-quadratic algorithm for the problem~\cite{Williams19}.
It is also known that the strong exponential time hypothesis (SETH) implies the Orthogonal Vectors hypothesis~\cite{Williams05}.
Thus, under \cref{thm:dkd1_quadratic_lower_bound}, the upper-bound of \cref{thm:dkd1_quadratic_upper_bound} is  (nearly) optimal.

\Paragraph{Bidirected $\Dyck_k\odot \Dyck_k$ reachability.}
Finally, we turn our attention to the general case of bidirected $\Dyck_k\odot \Dyck_k$ reachability.
The non-bidirected case is well-known to be undecidable~\cite{Reps00}, 
while it was recently shown~\cite{Li2021} that the bidirected case is $\NP$-hard, 
leaving its decidability open.
The following theorem resolves this open problem.

\smallskip
\begin{restatable}{theorem}{thmdkdkquadraticupperbound}\label{thm:dkdk_undecidable}
Bidirected $\Dyck_k\odot \Dyck_k$ reachability is undecidable.
\end{restatable}

In the following sections we present details of the above theorems.
To improve readability, in the main paper we present algorithms, examples, and proofs of all theorems.
To highlight the main steps of the proofs, we also present all intermediate lemmas;  many lemma proofs, however, are relegated to the appendix.


==> tables/tab_d1d1.tex <==
\begin{table}[]
\label{tab:d1d1}
\caption{\Andreas{TODO}}
\begin{tabular}{| c | c || c | c | c |}
\hline
\textbf{Benchmark} & \textbf{$n$} & \textbf{ID-SCCs} & \textbf{D-SCCs} & \textbf{Time (s)} \\ \hline \hline
antlr & 29831 & 26793 & 26825 & 28.91 \\ \hline
bloat & 36181 & 32693 & 32725 & 12.54 \\ \hline
chart & 67535 & 60787 & 60844 & 22.95 \\ \hline
eclipse & 30981 & 27812 & 27840 & 11.11 \\ \hline
fop & 61016 & 54671 & 54723 & 20.70 \\ \hline
hsqldb & 27494 & 24584 & 24610 & 10.44 \\ \hline
jython & 36162 & 31811 & 31845 & 17.59 \\ \hline
luindex & 28595 & 25610 & 25636 & 10.56 \\ \hline
lusearch & 29530 & 26417 & 26447 & 12.07 \\ \hline
pmd & 31333 & 28064 & 28093 & 12.32 \\ \hline
xalan & 27358 & 24498 & 24523 & 10.27 \\ \hline
\end{tabular}
\end{table}


==> tables/tab_dkd1.tex <==
% This table is results when flattening on "[", meaning "[" represents the D1 language

\begin{table}[]
\caption{\Andreas{Adam: TODO needs explanation of D1D1 - DkD1 column}}
\begin{tabular}{| c | c || c | c | c |}
\hline
\textbf{Benchmark} & \textbf{$n$} & \textbf{ID-SCCs} & \textbf{D-SCCs} & \textbf{Time (s)} \\ \hline \hline
antlr & 29831 & 27014 & 27015 & 9.05 \\ \hline
bloat & 36181 & 32946 & 32946 & 13.18 \\ \hline
chart & 67535 & 61158 & 61158 & 62.97 \\ \hline
eclipse & 30981 & 27999 & 28018 & 10.86 \\ \hline
fop & 61016 & 55012 & 55012 & 57.04 \\ \hline
hsqldb & 27494 & 24775 & 24776 & 8.19 \\ \hline
jython & 36162 & 32060 & 32062 & 21.09 \\ \hline
luindex & 28595 & 25809 & 25810 & 7.11 \\ \hline
lusearch & 29530 & 26655 & 26655 & 8.42 \\ \hline
pmd & 31333 & 28296 & 28297 & 9.10 \\ \hline
xalan & 27358 & 24689 & 24690 & 6.67 \\ \hline
\end{tabular}
\end{table}


% This table is results when flattening on "("

%Table when flattening on (\\

%\begin{table}[]
%\begin{tabular}{|l|l|l|l|l|l|l|l|}
%\hline
%Benchmark & N & ID-SCCs & ID reachable pairs & D-SCCs & D reachable pairs & D1D1 - DkD1 & Time (s) \\ \hline
%antlr & 29831 & 26825 & 1613938 & 26825 & 1613938 & 0 & 5.73852 \\ \hline
%bloat & 36181 & 32725 & 2290516 & 32725 & 2290516 & 0 & 5.4743 \\ \hline
%chart & 67535 & 60844 & 7240671 & 60844 & 7240671 & 0 & 19.1898 \\ \hline
%eclipse & 30981 & 27840 & 1796452 & 27840 & 1796452 & 0 & 5.05918 \\ \hline
%fop & 61016 & 54723 & 6536040 & 54723 & 6536040 & 0 & 17.7674 \\ \hline
%hsqldb & 27494 & 24610 & 1508413 & 24610 & 1508413 & 0 & 4.32403 \\ \hline
%jython & 36162 & 31845 & 4159201 & 31845 & 4159201 & 0 & 7.8304 \\ \hline
%luindex & 28595 & 25636 & 1569414 & 25636 & 1569414 & 0 & 4.36919 \\ \hline
%lusearch & 29530 & 26447 & 1614199 & 26447 & 1614199 & 0 & 6.14074 \\ \hline
%pmd & 31333 & 28093 & 1926461 & 28093 & 1926461 & 0 & 6.37289 \\ \hline
%xalan & 27358 & 24523 & 1446402 & 24523 & 1446402 & 0 & 4.42746 \\ \hline
%\end{tabular}
%\end{table}


==> tables/tab_merged.tex <==
\begin{table}[]
\label{tab:results_merged}
\caption{
Experimental results on $\Dyck_1\odot \Dyck_1$ and $\Dyck_k\odot \Dyck_1$ reachability.
In each case, ID-CCs denotes the number of connected components wrt the interleaved Dyck language,
while D-CCs denotes the number of connected components wrt the under-approximating Dyck language on the union alphabet.
%$n$ denotes the number of nodes in the input graph.
}
\begin{tabular}{| c | c || c | c | c || c | c | c |}
\hline
\textbf{Benchmark}  & \textbf{$n$} & \multicolumn{3}{c||}{$\Dyck_1 \odot \Dyck_1$} & \multicolumn{3}{c|}{$\Dyck_k \odot \Dyck_1$} \\ \hline
& & \textbf{ID-CCs} & \textbf{D-CCs} & \textbf{Time (s)} & \textbf{ID-CCs} & \textbf{D-CCs} & \textbf{Time (s)} \\ \hline \hline
antlr & 29831 & 26793 & 26825 & 28.91 & 27014 & 27015 & 9.05\\ \hline
bloat & 36181 & 32693 & 32725 & 12.54 & 32946 & 32946 & 13.18 \\ \hline
chart & 67535 & 60787 & 60844 & 22.95 & 61158 & 61158 & 62.97  \\ \hline
eclipse & 30981 & 27812 & 27840 & 11.11 & 27999 & 28018 & 10.86  \\ \hline
fop & 61016 & 54671 & 54723 & 20.70 & 55012 & 55012 & 57.04  \\ \hline
hsqldb & 27494 & 24584 & 24610 & 10.44 & 24775 & 24776 & 8.19  \\ \hline
jython & 36162 & 31811 & 31845 & 17.59 & 32060 & 32062 & 21.09 \\ \hline
luindex & 28595 & 25610 & 25636 & 10.56 & 25809 & 25810 & 7.11 \\ \hline
lusearch & 29530 & 26417 & 26447 & 12.07 & 26655 & 26655 & 8.42 \\ \hline
pmd & 31333 & 28064 & 28093 & 12.32 & 28296 & 28297 & 9.10 \\ \hline
xalan & 27358 & 24498 & 24523 & 10.27 & 24689 & 24690 & 6.67 \\ \hline
\end{tabular}
\end{table}

